NarrativeXL: A Large-scale Dataset For Long-Term Memory Models

We propose a new large-scale (nearly a million questions) ultra-long-context (more than 50,000 words average document length) reading comprehension dataset. Using GPT 3.5, we summarized each scene in 1,500 hand-curated fiction books from Project Gutenberg, which resulted in approximately 150 scene-level summaries per book. After that, we created a number of reading comprehension questions based on these summaries, including three types of multiple-choice scene recognition questions, as well as free-form narrative reconstruction questions. With 990,595 total questions, our dataset is an order of magnitude larger than the closest alternatives. Crucially, most questions have a known ``retention demand'', indicating how long-term of a memory is needed to answer them, which should aid long-term memory performance evaluation. We validate our data in four small-scale experiments: one with human labelers, and three with existing language models. We show that our questions 1) adequately represent the source material 2) can be used to diagnose a model's memory capacity 3) are not trivial for modern language models even when the memory demand does not exceed those models' context lengths. Lastly, we provide our code which can be used to further expand the dataset with minimal human labor.

==> emnlp2023-latex/tables/freeform_performance.tex <==
\begin{table*}[]

\begin{tabular}{p{0.2\linewidth}llll}
 & $R1_{F1}$ & $R2_{F1}$ & $RL_{F1}$ & $BertSCORE_{F1}$         \\ \hline
Baseline   & 0.522 (0.507, 0.537) & 0.261 (0.240, 0.282) &  0.408 (0.388, 0.427)          & 0.906 (0.903, 0.909) \\
GPT-3 (fine-tuned)                     & 0.504 (0.489, 0.518) & 0.236 (0.217, 0.255)& 0.384 (0.367, 0.402) & 0.9 (0.897, 0.903)   \\
GPT-4 no context  & 0.512 (0.497, 0.527) & 0.250 (0.23, 0.271) & 0.396 (0.378, 0.415) & 0.904 (0.901, 0.907) \\
\textbf{GPT-4 with context} & \textbf{0.576 (0.564, 0.588)}& \textbf{0.295 (0.287, 0.313)} & \textbf{0.422 (0.406, 0.438)} &  \textbf{0.913 (0.911, 0.915)}                  
\end{tabular}
\caption{Summary reconstruction performance. Baseline is obtained by comparing corrupted and uncorrupted summaries. Additionally, 95\% confidence intervals are given in parentheses (based on performance variation for 300 samples in the test set). Overall, GPT-4 with original book context performs best, while GPT-3 finetuned to correct summaries without knowing the book fails to find any shortcut solutions and performs near (below) baseline). Unsurprisingly, GPT-4 with no context fails to ``guess'' original book events.}
\label{tab:freeformperf}
\end{table*}

==> emnlp2023-latex/tables/summary_examples.tex <==

\begin{flushleft}
\begin{table*}
\begin{tabular}{ |p{0.3\linewidth}|p{0.3\linewidth}|p{0.3\linewidth}|  }
\hline
\multicolumn{3}{|c|}{Summary distortion} \\
\hline
Book Snippet & True Summary & False Summary \\
\hline
Salt-air and dazzling society kept all idea of penance from this vivacious young person. It was queer that Sit Twickenham should be at the seaside, instead of at Brookfield, wooing; but a man's physical condition should be an excuse for any intermission of attentions. "Now that I know him better," wrote Adela, "I think him the pink of chivalry; and of this I am sure I can convince you, Bella, C. will be blessed indeed; for a delicate nature in a man of the world is a treasure. He has a beautiful little vessel of his own sailing beside us [...]



 & The excerpt describes Adela and Arabella's different experiences during the yachting excursions. Adela is having a great time and writes to Arabella about the fun they are having. Arabella, on the other hand, is miserable and writes to Adela about the mundane daily events at Brookfield. The Hon. Mrs. Bayruffle accompanies the ladies on the yacht and Adela admires her social skills but realizes that society is not everything. The excerpt also touches on the idea that when people experience a great fall, they rarely indulge in melancholy until they can take it as a luxury. & The excerpt describes two friends, Adela and Arabella, taking a walk in the countryside. Adela is awestruck by the natural beauty around them and tells Arabella about the great time they are having. Arabella, however, is unimpressed and complains to Adela about the lack of proper civilization out here. The Hon. Mrs. Bayruffle joins the ladies for the walk and Adela learns a valuable lesson about the importance of solitude. The excerpt also touches on the idea that adversity reveals the true strength of a person's character. \\
\hline



\end{tabular}

\caption{\footnotesize True and distorted summary example. Crucially, we aimed to keep the setting the same, only changing the described events. This way, we hope to encourage models trained on our data to precisely remember book events rather than style, characters, or setting.}

\end{table*}\label{tab:truefalsesummaries}

\end{flushleft}
